Koo-Fu CLIP: Closed-Form Adaptation of Vision-Language Models via Fukunaga-Koontz Linear Discriminant Analysis

Visual-language models such as CLIP provide powerful general-purpose representations, but their raw embeddings are not optimized for supervised classification, often exhibiting limited class separation and excessive dimensionality. We propose Koo-Fu CLIP, a supervised CLIP adaptation method based on Fukunaga-Koontz Linear Discriminant Analysis, which operates in a whitened embedding space to suppress within-class variation and enhance between-class discrimination. The resulting closed-form linear projection reshapes the geometry of CLIP embeddings, improving class separability while performing effective dimensionality reduction, and provides a lightweight and efficient adaptation of CLIP representations. Across large-scale ImageNet benchmarks, nearest visual prototype classification in the Koo-Fu CLIP space improves top-1 accuracy from 75.1% to 79.1% on ImageNet-1K, with consistent gains persisting as the label space expands to 14K and 21K classes. The method supports substantial compression by up to 10-12x with little or no loss in accuracy, enabling efficient large-scale classification and retrieval.

==> tables/ablation_l2_21k.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{crrrrr}
        \toprule
        Space & & \multicolumn{2}{c}{Top-1} & \multicolumn{2}{c}{Top-5} \\
        $f(\cdot)$ & \multicolumn{1}{c}{$\lambda$} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Val.} & \multicolumn{1}{c}{Clean} & \multicolumn{1}{c}{Val.} \\
        \midrule
        (--) &  --- & 53.48 & 45.08 & 83.04 & 74.32 \\
        \midrule
        (21K) & \textless{74k} & --- & --- & --- & --- \\
        (21K) &  75k & 53.42 & 45.03 & 82.94 & 74.19 \\
        (21K) & 100k & 53.46 & 45.08 & 82.97 & 74.23 \\
        %(21K) & 125k & 53.47 & 45.09 & 83.00 & 74.28 \\
        (21K) & 150k & 53.48 & 45.08 & 83.04 & 74.32 \\
        %(21K) & 200k & 53.44 & 45.06 & \textbf{83.06} & 74.33 \\
        (21K) & 250k & 53.44 & 45.07 & \textbf{83.06} & 74.34 \\
        (21K) & 500k & \textbf{53.49} & 45.10 & 83.05 & \textbf{74.36} \\
        (21K) & 750k & 53.48 & \textbf{45.11} & 82.98 & 74.29 \\
        (21K) &   1M & 53.46 & 45.09 & 82.93 & 74.28 \\
        \bottomrule
    \end{tabular}
    \caption{
    {\bf Regularization ablation for 21K-stats transformation, setting with distractors (21K).}
    Similar to the 1K ablation, accuracy remains robust across a broad range of $\lambda$.
}
\end{table}
